OFA: Unifying Architectures, Tasks, and Modalities Through a Simple Sequence-to-Sequence Learning Framework

In this work, we pursue a unified paradigm for multimodal pretraining to break the scaffolds of complex task/modality-specific customization. We propose OFA, a Task-Agnostic and Modality-Agnostic framework that supports Task Comprehensiveness. OFA unifies a diverse set of cross-modal and unimodal tasks, including image generation, visual grounding, image captioning, image classification, language modeling, etc., in a simple sequence-to-sequence learning framework. OFA follows the instruction-based learning in both pretraining and finetuning stages, requiring no extra task-specific layers for downstream tasks. In comparison with the recent state-of-the-art vision & language models that rely on extremely large cross-modal datasets, OFA is pretrained on only 20M publicly available image-text pairs. Despite its simplicity and relatively small-scale training data, OFA achieves new SOTAs in a series of cross-modal tasks while attaining highly competitive performances on uni-modal tasks. Our further analysis indicates that OFA can also effectively transfer to unseen tasks and unseen domains. Our code and models are publicly available at https://github.com/OFA-Sys/OFA.

==> table/finetuning_details.tex <==
\begin{table*}[t]
\caption{Hyper-parameters for finetuning on GLUE.}
\vskip 0.15in
\centering
\begin{adjustbox}{max width=1.\textwidth}
\begin{tabular}{@{\extracolsep{\fill}}lcccccccc}
\toprule

  &COLA
  &SST-2 
  &RTE
  &MRPC
  &QQP
  &MNLI
  &QNLI
  &WNLI
  \\
  \midrule
  Training Steps
  &1334
  &
  &
  &
  &
  &
  &
  &
  \\
  Warmup Steps
  &80
  &
  &
  &
  &
  &
  &
  \\
  Batch Size
  &64
  &
  &
  &
  &
  &
  &
  &
  \\
  Learning Rate
  &6e-5
  & 
  &
  &
  &
  &
  &
  \\
  Weight decay
  &0.01
  & 
  &
  &
  &
  &
  &
  \\
  Enc. Stoch. Depth
  &0.1
  & 
  &
  &
  &
  &
  &
  \\
  Dec. Stoch. Depth
  &0.1
  & 
  &
  &
  &
  &
  &
  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:glue-hyper}
\end{table*}
